Leveraging Visual Tokens for Extended Text Contexts in Multi-Modal Learning

Training models with longer in-context lengths is a significant challenge for multimodal model due to substantial GPU memory and computational costs. This exploratory study does not present state-of-the-art models; rather, it introduces an innovative method designed to increase in-context text length in multi-modality large language models (MLLMs) efficiently. We present Visualized In-Context Text Processing (VisInContext), which processes long in-context text using visual tokens. This technique significantly reduces GPU memory usage and floating point operations (FLOPs) for both training and inferenceing stage. For instance, our method expands the pre-training in-context text length from 256 to 2048 tokens with nearly same FLOPs for a 56 billion parameter MOE model. Experimental results demonstrate that model trained with VisInContext delivers superior performance on common downstream benchmarks for in-context few-shot evaluation. Additionally, VisInContext is complementary to existing methods for increasing in-context text length and enhances document understanding capabilities, showing great potential in document QA tasks and sequential document retrieval.

==> figures/6-overall_fuyu.tex <==
\begin{figure}[ht]
    \centering
    \begin{minipage}{0.35\textwidth}
        \centering
    \includegraphics[width=\linewidth]{figures/src/main_ppl_fuyu.eps}
    \end{minipage}\hfill
    \begin{minipage}{0.62\textwidth}
        \centering
        \caption{\small The main pipeline is based on Fuyu~\cite{adept_fuyu8b}.
        What's different is we introduce an additional text image.
        During pre-training, the rendered text image and original image is also alternatively.
        The DCSE is preserved.
        We show one image-text pair here for simplicity.}
        \label{fig:overall_fuyu}
    \end{minipage}
\end{figure}


==> tables/idelics_ablation.tex <==
\begin{table*}[h]
\centering
% \footnotesize
%\scriptsize
\scalebox{.95}{
\begin{NiceTabularX}{\linewidth}{lx{34}ccccccccccc}
\CodeBefore
\rowlistcolors{1}{background,background,background,background,background,background,background,background,softblue,softblue,softblue,background,background,background,softblue,softblue,softblue,background,background,background,background,background,background,softblue,softblue,softblue}
\Body
  % \footnotesize
%  \scriptsize
    \bf Method  & \bf Text Source & \bf Parameter & \bf Tokens$\downarrow$&\bf T-Shots  & \multicolumn{4}{c}{\bf VQA}  \\
    & & & &  & ok-vqa & textvqa & vizwiz & vqav2  \\
    \midrule
    \bf \multirow{3}{*}{\parbox[c]{2cm}{IDELICS3B Baseline~\cite{obelics}}$\dag$}  &  \multirow{3}{*}{\makecell{Raw \\ Text}} & \multirow{3}{*}{1.4B/3.2B} & 10
    & 0&  \\
    &&&50& 4 & \\
    &&&142& 32 &  \\
    \hline
    \bf \multirow{3}{*}{\parbox[c]{.5cm}{\ModelName}}   &  \multirow{3}{*}{\makecell{Rendered \\ Image}}  & \multirow{3}{*}{1.0B/3.0B} & 0
    & 10& 11.2 & 15.8 & 5.4 & 33.6  \\
    &&&10& 4 & 17.2 & 21.8 & 9.73 & 33.2   \\
    &&&10& 32 & 21.3 & 22.6 & 11.5 & 35.8   \\
    \bottomrule
\end{NiceTabularX}
}
    \caption{
    \textbf{Comparison Across Various In-context Length without image input}.
    Here we show \textbf{the shots means in-context example without image.}
     $\dag$ means our implementation on 180M data.
    }
    \label{tab:sota}
\end{table*}
